Orientation and microstructure in sheared Brownian suspensions of anisotropic dicolloidal particles

Orientation and microstructure are investigated in sheared Brownian suspensions of hard dicolloidal particles, with the dicolloids modeled as two fused spheres of varying radii and center to center separations. Two different particle shapes named homonuclear (aspect ratio 1.1) and fused-dumbbells (aspect ratio 1.5) were considered. Hydrodynamic interactions between the particles were computed with a modified lubrication model called Fast Lubrication Dynamics. Studies were conducted for a wide range of volume fractions between $0.3 \leq \phi \leq 0.5$ and P\`{e}clet numbers between $0 \leq Pe \leq 1000$. The microstructure was found to be disordered at all volume fractions, though signatures of weak string like ordering were evident particularly in $\phi=0.5$ homonuclear suspensions at intermediate to high shear rates ($Pe$ in the range 10-100). Complex orientation behavior was observed as a function of shape, shear rates, and volume fractions. At very low shear rates, random orientation distribution was observed in all cases. At the highest shear rates, orientation distribution in suspensions of homonuclear particles exhibited a shift towards an alignment with the vorticity axis at all volume fractions, while in suspensions of fused-dumbbells it exhibited a shift away from the vorticity axis at low volume fractions and a negligible shift at higher volume fractions. The orientation behavior is further characterized by examining the orientation distribution in the velocity--gradient plane -- in this case an increased particle alignment with the velocity axis is generally observed with increasing volume fractions, but not universally with increasing shear rates. Mechanistic origins for the complex orientation behavior as a function of shear rate, volume fraction, and particle shape is described.

==> results.tex <==
\section{Results}
\subsection{Microstructure}\label{sec:struct}
%
We begin by reviewing the equilibrium microstructure for particle
suspensions in quiescent conditions, which establishes a standard
for comparison for the microstructure in sheared suspensions.
Suspensions of spheres in a quiescent system at equilibrium exist
in a fluid like state below $\phi=0.494$ and in a face centered
cubic (FCC) state above a volume fraction of $\phi=0.545$;
experimentally a random stacking of hexagonally close packed layers
could also be observed \citep{pusey89,solomon08}.
The volume fraction $\phi=0.494$ is commonly known as the freezing
point, while the volume fraction $\phi=0.545$ is known as the
melting point. Between these two volume fractions, coexisting
fluid and FCC phases are found. The equilibrium microstructure for
hard-dicolloids with fore-aft symmetry has been characterized via
numerical simulations \citep{vega92b}. The freezing and melting
transitions for dicolloids with $c/a=0.2$ (homonuclear) were found
to occur at approximately $\phi=0.4945$ and $\phi=0.543$
respectively, while for dicolloids with $c/a=1.0$
(fused-dumbbell), the same two transitions were found to occur at
approximately $\phi=0.6013$ and $\phi=0.6463$ (these data were read
off from Fig. 3 in the previous reference). Moreover, the
ordered phase at the freezing transition is orientationally
disordered (plastic crystal) in suspensions of dicolloids with
$c/a=0.2$, while it is orientationally ordered in suspensions of
dicolloids with $c/a=1.0$. In simulations, the ordered phase is
typically observed at volume fractions above the melting
transition \citep{speedy97}. The maximum volume fraction
investigated in the present work is $\phi=0.55$, hence the
equilibrium microstructure is expected to be disordered in
fused-dumbbell particle suspensions at all volume fractions
studied here, while an ordered microstructure is expected in
suspensions of spheres and homonuclear particles at $\phi=0.55$.
\modify{It is also appropriate to note here that a nematic phase is not expected
for dicolloidal particles. This is due to the fact that the degree of anisotropy
  of dicolloids is small, while the nematic phase is stable only
at higher aspect ratios. As an example, for spherocylinders, the nematic phase becomes
stable at an aspect ratio of 4.7 \citep{bolhius97}. Another interesting
phase shown by dicolloidal particles at equilibrium is the aperiodic solid phase
(degenerate crystals) at densities intermediate to that where the fluid
and the crystalline solid phases are stable \citep{woj91,woj92,liddell08}.
This phase, though, is stable only for higher aspect ratio dicolloids
in three dimensions with $c/a > 1.84$ \citep{djikstra08}. This aperiodic
phase is therefore not expected for particle shapes investigated in this study.}


When a suspension of spheres is sheared, its microstructure goes
through a series of transitions as characterized by
\citet{chow95}. At high shear rates where Brownian effects are
negligible, a disordered state is typically obtained in
suspensions of spheres \citep{chow95} comparable to the
non-Brownian systems studied in this work. Very little is known
about the microstructure of dicolloids under shear.
\citet{mock07} studied charge-stabilized dicolloids at low shear
rates for volume fraction of $\phi=0.42$, where all dicolloids
had a small degree of anisotropy ($\leq$ homonuclear). They
observed a series of microstructural transitions with increasing
shear rate analogous to the results for suspensions of spheres
with comparable electrostatic potential.  These authors did not
study the high shear limit, however a disordered state is
expected comparable to the results for spheres.

We turn to the present results for the microstructure of
suspensions for four different particle shapes - spheres,
homonuclear, small-bump and fused-dumbbell dicolloids.  To
characterize the microstructure, we employ pair distribution
functions (PDF) in the three planes of interest, designated as
front view (flow-gradient plane $\equiv$ $g({x},{y})$), top view
(flow-vorticity plane $\equiv$ $g({x},{z})$) and end view
(vorticity-gradient plane $\equiv$ $g({z},{y})$)  (See Fig.
\ref{fig:views}). As an example, the two dimensional function,
$g({x},{y})$ is obtained from the full three dimensional PDF
$g({x},{y},{z})$ by integrating over a slice of one particle
diameter along the $z$ direction as
\begin{equation}
g({x},{y}) = \frac{1}{2a} \int_{-a}^{+a} g({x},{y},{z}) dz
\end{equation}

For all volume fractions below $\phi \leq 0.5$ studied in this
work, a disordered state was obtained for all particle shapes.
This is similar to the behavior at equilibrium, though the
detailed characteristics of the microstructure are quite
different. The PDF's for the front view for all four particle
shapes are shown in Fig.\ref{fig:50_gxy} for two representative
volume fractions: $\phi=0.1$ and $\phi=0.5$. For dicolloidal
particles, the PDF is computed from the correlations between the
center-of-mass of the particles. At low volume fractions (e.g.
$\phi=0.1$), a disordered state is obvious from the PDFs. As the
volume fraction is increased, features of weak string like
ordering begin to emerge in suspensions of spheres and dicolloids
with small degree of anisotropy (small-bump and homonuclear) for
$\phi > 0.4$. The presence of weak string like characteristic in
the microstructure is clearly seen in the PDFs
(Fig.\ref{fig:50_gxy}) at $\phi=0.5$, though no long range order
is present at that volume fraction. For fused-dumbbells, no
significant sign of string like ordering is observed.  An
interesting feature of the PDF is the lack of fore-aft symmetry,
which can be attributed to the presence of non-hydrodynamic
interactions - short range repulsive forces in this study
\citep{brady97}. In a suspension with purely hydrodynamic
interactions, the reversibility of Stokes flow combined with the
fore-aft symmetry of the geometry and imposed flow field leads to
fore-aft symmetric pair distribution function
\citep{koch97}. The presence of non-hydrodynamic interactions
break the reversibility and consequently may lead to fore-aft
asymmetric PDF with rheological consequences, i.e. non-Newtonian
effects \citep{brady97}.

Moving to higher volume fraction, we present the microstructure
for $\phi=0.55$. At this volume fraction, a one-dimensional long
range string like ordering was observed for spherical,
homonuclear, and small-bump particle suspensions. Marginal hints
of layering are observed for fused-dumbbells, however the
suspensions are primarily disordered. The string like nature for
the ordered systems is shown in the PDF's shown in
Fig.\ref{fig:55_gxyz}. In the front and top views, horizontal
bands can be seen, where the central band corresponds to the home
string of the reference particle. The two PDF's show no
correlation between particle positions in different bands, which
is characteristic of strings and rules against the presence of
ordered layers.  In the end view, hexagonal packing of the strings
can be seen. \citet{brady2002} observed similar string like
ordering in their Stokesian Dynamics simulations of non-Brownian
spheres at $\phi=0.55$. As noted earlier, in experiments at high
shear rates where the effect of Brownian or interparticle
interactions are negligible (except in a thin boundary layer
\citep{brady97}), a disordered state is usually obtained. In some
experiments, the microstructure at high volume fractions and at
high shear rates has been shown to fluctuate with time with the
appearance and disappearance of well defined maxima in scattering
patterns \citep{chen94}. Similarly, \citet{wagner96prl} observed  a
metastable crystalline state after the cessation
of shear from a shear thickened disordered state ($\phi=0.48$).
This led to the suggestion of latent order in the shear thickened
state which is not readily apparent in scattering measurements.
Both these experimental observations are consistent with the
observation of order in the present numerical simulations.
Finally, the disordered microstructure in the fused-dumbbell
suspensions at $\phi=0.55$ is consistent with equilibrium results
which require much higher volume fractions ($\phi> 0.6$) for
freezing or melting transitions.



\subsection{Rheology}\label{sec:rheo}
\subsubsection{Viscosity}
The viscosity for all particle shapes as a function of volume
fraction is plotted in Fig. (\ref{fig:mu}a) and tabulated in Tables
(\ref{tb:mu_sp}) and (\ref{tb:mu_all}). \modify{ The statistical error in the
average viscosity is less than $0.1\%$ for all particle shapes
and at all volume fractions, while the statistical error
in the average normal stress differences is less than $1\%$.
The symbol size in the previous figure and in the figures discussed
in the following section is at least an order of magnitude larger
than the corresponding error, and hence these are not shown
on these plots.}
In figure (\ref{fig:mu}a), we also show the
viscosity for suspensions of spheres reported for Stokesian
Dynamics simulations by \citet{brady2002}. Our results are in
excellent agreement with the earlier study though a different
algebraic form of interparticle force is used in the two studies. The
range of the interparticle force is approximately equal
($10^{-3}\times$radius). In comparison to experimental values,
omitted here for clarity, the simulated values are smaller at high
volume fractions \citep{brady2002}. However, as noted in the
earlier study, this discrepancy can be attributed to the range and
strength of the interparticle force employed in the simulation.
The contribution to viscosity from interparticle forces for
suspensions of spheres is tabulated in Table \ref{tb:mu_spb}. As
can be seen, this contribution is negligible in comparison to the
overall viscosity. Nonetheless, the distribution of smallest gaps
in the system is strongly affected by the interparticle force,
which in turn affects the hydrodynamic contribution to viscosity.
In general, a greater hydrodynamic viscosity is expected when the
range of interparticle interaction is reduced, as that leads to
smaller gaps and larger lubrication forces \citep{viera02,brady2002}.

Fig. (\ref{fig:mu}a) provides an interesting comparison of viscosity
for different particle shapes. At the lowest volume fractions,
the fused-dumbbells have the highest viscosity, which can be
attributed to higher intrinsic viscosity ($[\mu]$ in Table \ref{tb:sing_loc}).
In non-dilute suspensions ($0.2 \leq \phi \leq
0.5$) however, the fused-dumbbells show the smallest viscosity among dicolloids
(see Tables \ref{tb:mu_sp} \& \ref{tb:mu_all}). \modify{These trends are
readily observed in Fig. (\ref{fig:mu}b), where we plot the
ratio of suspension viscosities of dicolloids and
spheres at the same volume fraction.} A similar trend
was observed in the infinite frequency viscosity for these
particles \citep{kumar09,kumar10}. The slower divergence in viscosity
with volume fraction can be attributed to a higher value for
random close-packed volume fraction (RCP). To first
approximation, RCP for dicolloids may be estimated by
considering values for spheroids with the same aspect ratio.
\citet{chaikin04} showed that a prolate spheroid with an aspect
ratio of approximately 1.5 has the largest RCP with this maxima
being $\phi_{RCP} \approx 0.71$ (compared to $\phi_{RCP}\approx
0.64$ in suspensions of spheres). The fused-dumbbell particle
with an approximate aspect ratio of 1.5 may be expected to have
the highest RCP among dicolloids studied here. A larger RCP
implies a slower divergence of viscosity with more free volume
at a given volume fraction. Note that the divergence of the
infinite shear viscosity does not necessarily occur at
$\phi_{RCP}$. Flow induced microstructural distortions may lead
to divergence at higher volume fractions as in the results of
\citet{vander89} for spheres. While a strict correspondence may
not always be inferred, a general trend is observed with higher
volume fraction for viscosity divergence associated with
increasing $\phi_{RCP}$. As a final point of interest in
Fig.\ref{fig:mu}, at $\phi=0.55$, all particles except
fused-dumbbells exhibit a slight decrease in viscosity with
increasing  $\phi$. This is associated with the string-like
ordered microstructure.


\subsubsection{Normal Stress Differences}\label{sec:normstress}
In suspensions with statistically symmetric microstructure and
purely hydrodynamic interactions, normal-stress differences are
expected to be zero. This follows from the symmetry of the imposed
flow, the particle distribution function, and the reversibility of
Stokes flow \citep{koch97}, though such systems are known to be chaotic
\citep{pine05}. The presence of the repulsive force
breaks the reversibility condition and leads to a microstructure
lacking fore-aft symmetry as was shown in section
(\ref{sec:struct}). In addition to the positional asymmetry, an
asymmetry in the orientational distribution function is also
expected \citep{koch97}. Asymmetry in the orientational
distribution function of non-spherical particles may lead to
non-zero mean normal stress differences at the single particle
level, however these may be insignificant for particles with small
degree of anisotropy.

We begin by presenting normal stress data for our numerical
simulations for suspensions of spheres in Table \ref{tb:mu_sp}. At
$\phi \leq 0.5$ where the microstructure is disordered, both the
first and the second normal stress differences are negative. We
have compared the normal-stress differences in this study with
other numerical and experimental works in Fig. \ref{fig:N1} and
Fig. \ref{fig:N2} for the first and second normal stress
differences respectively. Each figure includes normal stress data
plotted on both linear and logarithmic axes. Results for dicolloid
particles are also included in these figures. Normal stress
differences in this work agree well with the numerical results of
\citet{brady2002}. Good agreement for the first normal-stress
difference is obtained with the experimental work of
\citet{nott2003}, but the numerical simulations give second normal
stress differences a factor of two smaller than experiments.
\citet{brady2002} attributed this difference to the presence of
friction, while \citet{nott2003} attributed this to the effect of
the interparticle force used in simulations. The definitive
explanation for this consistent discrepancy between simulations
and experiments remains elusive. In the data for normal stress differences in Table
\ref{tb:mu_sp}, we also include the specific contributions due to
interparticle forces in suspensions of spheres. These show that
the direct contribution is negligible for volume fractions up to
$\phi=0.5$ where the microstructure is disordered. However, the
interparticle forces have an indirect effect by breaking the
reversibility of Stokes flow and by controlling the distribution
of small interparticle gaps where large hydrodynamic lubrication
forces play a major role. At $\phi=0.55$, an ordered
microstructure arises and both the normal stress differences
become positive. A change to positive first normal stress
difference is typically observed in experiments at high volume
fractions and high shear rates in conjunction with a rapid
increase in viscosity indicating an approach to jamming
\citep{hebraud05}. While no jamming is observed here, the ordered
microstructure is highly anisotropic leading to the change of sign
in the normal stress differences. It is interesting to note that
the interparticle force contribution to normal stress differences
can be significant in the ordered states at $\phi=0.55$ (Table
\ref{tb:mu_sp}).

Results for normal stress differences in suspensions of
dicolloidal particles are presented in Table 4 and plotted in
Figures \ref{fig:N1} and \ref{fig:N2} discussed above. Similar
to the results for spheres, both the first and second normal
stress differences were negative for $\phi \leq 0.5$. The
magnitudes of the normal stress differences were typically close
to those of spheres. In terms of absolute value, the first
normal stress difference was typically higher in homonuclear
particle suspensions, while the second normal stress difference
was typically higher in fused-dumbbell particle suspensions. For
fused-dumbbells, note that the second normal stress difference
can be several times higher than the first normal stress
difference at high volume fractions (e.g. $\phi=0.5$). This is
in contrast to the behavior observed in suspensions of spheres
and other dicolloids where the two are of comparable magnitude.
At the highest volume fraction ($\phi=0.55$), the first normal
stress difference changes sign and becomes positive for
homonuclear and small-bump particles similar to the result for
spheres.  This is likely due to the ordering transition in these
suspensions. For fused-dumbbells, the first normal stress
difference remains negative at $\phi=0.55$; it decreases in
magnitude over the corresponding value at $\phi=0.5$.  This
shows a shift towards positive values which is similar to that
for other particle shapes in this work and for experimental
results at high volume fractions and high shear rates noted
above \citep{hebraud05}.

\subsection{Orientation}\label{sec:oc}
In this section, we begin with a discussion of orientation
distribution in suspensions of anisotropic particles at
infinite dilution. \modify{The limit of infinite dilution
is defined here as a system of non-interacting, essentially isolated particles
with $\phi \rightarrow 0$.} This is followed by a discussion of the effects of
particle interactions on the orientation distribution in suspensions
at finite volume fractions.

\subsubsection{Orientation at infinite dilution}\label{sec:resulta}
\citet{jeffery22} showed that a spheroid in a shear flow at low
Reynolds number would rotate in a periodic orbit whose 
geometry depends on its initial orientation. The Jeffery orbits
comprise an infinite family of orbits characterized by a single
parameter ``$C$" (see Eq. \ref{eq:jeffb} below). In an extension
of Jeffery's result, \citet{bretherton62} showed that axisymmetric
bodies of more general shape execute Jeffery orbits similar to
spheroids with an effective aspect ratio $r_e$ replacing the
aspect ratio $r_p$ of the spheroid. For  high aspect ratio
cylindrical fibers, the ratio $r_e/r_p$ decreases with increasing
particle aspect ratio $r_p$. Typical values of $r_e/r_p$ lie
between $0.6-0.7$ for $r_p <100$ \citep{koch2000}. Effective
aspect ratios for dicolloidal particles are presented below.

For an arbitrary axisymmetric body, its orientation may be
specified by spherical coordinates ($\varphi,\theta$) where
$\theta$ measures the angle between the particle axis and $z$ axis
and $\varphi$ is angle measured from the $y$ axis in the $xy$
plane. The evolution of the orientational angles
($\varphi,\theta$) in shear flow with time $t$ is given by (see
Fig. \ref{fig:jeffery})
\begin{subequations}\label{eq:jeff}
\begin{equation}\label{eq:jeffa}
\tan\varphi = r_e \tan \left(\displaystyle \frac{\dot{\gamma} t}{r_e + 1/r_e} + \kappa \right)
\end{equation}
\begin{equation}\label{eq:jeffb}
\tan \theta =  \displaystyle \frac{C r_e }{ \sqrt{r_e^2\cos^2 \varphi + \sin^2 \varphi}}
\end{equation}
\end{subequations}
Here $\kappa$ denotes the initial phase and $C$ is the orbit
constant. Two limiting values are $C=0$ for particles aligned with
the vorticity axis of the flow ($z$) and $C=\infty$ for particles
aligned in the velocity-gradient plane ($x-y$). Both $C$ and
$\kappa$ are completely determined by the initial orientation. The
period of rotation $T$ in the Jeffery's orbit follows from Eq.
(\ref{eq:jeffa}) and is given by
\begin{equation}\label{tperiod}
T = \frac{2\pi}{\dot{\gamma}} \left( r_e + \frac{1}{r_e} \right)
\end{equation}
Note that the orbit period depends solely on the particle shape and
is independent of the orbit constant. For dicolloidal particles,
numerical simulations were conducted to determine the orbit
periods and hence to find the effective aspect ratio $r_e$ using
Eq. (\ref{tperiod}).  These computations yield an effective aspect
ratio of 1.0868, 1.0967, and 1.5075 for the homonuclear,
small-bump, and fused-dumbbell particles respectively (Table
\ref{tb:re_sxx}). By comparison, the aspect ratios based purely on
geometry give 1.1, 1.1 and 1.5 respectively, quite close to the
values obtained from the Jeffery's orbit calculation.

To characterize the statistical distribution of particle
orientations in a suspension, we define an orientational order
parameter relative to each coordinate axis $i$ as the average
over all particles of
\begin{equation}\label{eq:Sii}
S_{ii} = \frac{3}{2}n_i n_i - \frac{1}{2}
\end{equation}
Here $n_i$ designates the component of the unit vector along the
particle symmetry axis (the director $\mathbf{n}$) with $i$
taking values $x,y,z$. For a random dispersion $S_{ii}=0$; for
perfect alignment of particles with axis $i$, $S_{ii}=1.0$; and
for particles aligned in the plane perpendicular to $i$,
$S_{ii}=-0.5$. Even in the absence of particle interactions, a
particle immersed in a shear flow exhibits preferred average
orientation due to the non-uniform rate of rotation in the
orbits.  In particular, particles spend a greater portion of the
orbital period aligned near the velocity-vorticity plane
compared with the gradient-vorticity plane.


To compute the orientational order parameter for a suspension at
infinite dilution with non-interacting particles, one must specify the initial distribution of
particles into orbits as specified by $C$. There are two simple
ways which can be used to compute this initial
distribution. In the first scheme, one assumes that the director
of the particle is initially uniformly distributed in the
($\varphi,\theta$) space, which then dictates the statistical
distribution of $C$ as determined from Eq. (\ref{eq:jeffb}).
Alternatively, in the presence of an asymptotically weak rotary
diffusivity, an arbitrary initial distribution will evolve into a
determinate distribution of orbit constants as given by
\citet{leal71}. For the modest particle aspect ratios investigated
in this work, the two methods lead to nearly identical
distributions; hence for simplicity, we assume an initially
isotropic distribution. The time average distribution yields the
probability distribution shown in Fig.\ref{fig:cb0}. For
convenience, we define a normalized orbit constant $C_b$
\begin{equation}
C_b = \frac{C}{C+1}
\end{equation}
where $C_b$ varies between $0$ and $1$ as $C$ varies from $0$ to
$\infty$.  The value $C_b=0$ corresponds to alignment with the
vorticity axis, while $C_b=1$ corresponds to alignment in the
velocity-gradient plane. In Fig.\ref{fig:cb0}, $p(C_b)$ gives the
probability of finding a particle with a given $C_b$ with
normalization:
\begin{equation}
\int_{0}^{1} p(C_b) dC_b = 1
\end{equation}
For later use, we define the mean orbit constant $C_b^m$  as
follows
\begin{equation}
C_b^m = \int_{0}^{1} p(C_b)\,C_b \,dC_b
\end{equation}
which is the first moment of the probability distribution
function $p(C_b)$.  This parameter will prove most useful in
characterizing the distribution of particle orientations.

For suspensions at infinite dilution, each particle executes a
Jeffery orbit with specified orbit constant $C_b$. Once the
distribution into orbits $p(C_b)$ is specified, the overall mean
orientational order parameter (\ref{eq:Sii}) is easily obtained
by time averaging over the period of the orbit for each $C_b$
and averaging over the distribution of orbit constants. The mean
order parameters are tabulated in Table \ref{tb:re_sxx} for all
particle shapes considered in this study. Dicolloids with small
degree of anisotropy, i.e. homonuclear and small-bump particles,
show a modest increase in the orientational order parameter in
the flow direction $S_{xx}$, primarily at the expense of the
orientational order parameter in the gradient direction
$S_{yy}$. By comparison, fused-dumbbells show a significant
increase in $S_{xx}$ (alignment with velocity axis) which is
expected due to its larger degree of anisotropy. We note that
the orientational order parameter for the vorticity axis
$S_{zz}$ is negligibly affected by rotations in Jeffery's orbit
for particles considered here.

\subsubsection{Orientation distribution at finite concentration}
In this section, we present the main computational results of this
study for average orientation distributions in sheared suspensions
of dicolloidal particles at finite concentrations. We focus on
average distributions here and investigate dynamics and
micromechanics in the next section \ref{sec:discuss}.  To
characterize the statistical distribution of particle orientations
in the suspensions, we choose two measures based on the
definitions of the section \ref{sec:resulta} above.  The first is
the mean orientation order parameter $S_{ii}$ which gives a direct
measure of the degree of particle orientation relative to the
velocity-gradient-vorticity axes.  The second measure is based on
the mean orbit constant $C_b^m$ as a measure of the probability
distribution function $p(C_b)$. At finite volume fraction,
particles no longer execute perfect Jeffery's orbits owing to
particle interactions.  Nonetheless, we may use the orbit
parameter $C_b$ to characterize a particle's instantaneous
orientation and compute the rate of change of orbit parameter to
characterize the effect of particle interactions.  Previously, we
have computed the mean orbit constant $C_b^m$ for infinite
dilution, and we now define $\Delta C_b^m$ as the difference of
mean orbit constant relative to infinite dilution.  Positive
values of $\Delta C_b^m$ indicate an increase in $C_b^m$ and a net
shift of orientation away from the vorticity axis and toward the
velocity-gradient plane.  Negative values of $C_b^m$ indicate a
shift in orientation toward the vorticity axis.  As this quantity
is defined relative to infinite dilution, it captures the net
influence of particle interactions, in effect measuring the
departure from the non-uniform probability distribution shown in
Fig. (\ref{fig:cb0}) associated with the single particle
Jeffery orbit. Fig. (\ref{fig:cb_avg}) shows $\Delta C_b^m$ as a
function of volume fraction for each of the three dicolloid
particle shapes. Fig. (\ref{fig:oc_all}) shows the corresponding
orientation order parameters $S_{xx}, S_{yy}, S_{zz}$ as a
function of volume fraction for each of the three particle shapes.
\modify{The statistical error in the average orbit constant as well as
in the average orientation order parameter is less than
$0.1\%$ for all cases. The errors are, therefore, considerably smaller than
the symbol sizes in the previous two figures.}

We begin our discussion of these figures by considering the
results for homonuclear particles. By definition, $\Delta
C_b^m=0$ at infinite dilution. At low volume fractions up to
($\phi=0.05$), there is a clear increase in the mean orbit
constant with positive $\Delta C_b^m$.  This reflects a net
change in orientation moving away from the vorticity axis.  This
is accompanied by an increase in the orientational order
parameter along the $x$ and $y$ axis with a corresponding
decrease in orientational order along the $z$ direction. With
increasing volume fraction above $\phi=0.05$, there is a
monotonic decrease in $\Delta C_b^m $ with increasing $\phi$
representing a shift in orientation toward the vorticity axis.
This is reflected in the monotonic increase in order parameter
$S$ along $z$ axis.  The overall behavior of homonuclear
particles is intriguing as it shows that particle interactions
initially favor movement away from the vorticity axis but shift
at higher volume fraction and favor movement toward the
vorticity axis.


Next, we turn our attention to small bump particles.  In contrast
to the homonuclear particles, there is negligible change in
$C_b^m$ up to $\phi=0.10$. This is confirmed by the plots for the
orientational order parameters.  For higher volume fractions, the
small bump particles exhibit orientation behavior similar to the
homonuclear particles; that is they show a negative $\Delta C_b^m
$ and a shift toward the vorticity axis. On the other hand,
despite a shift toward the vorticity axis and increase in $S_{zz}$
at higher volume fractions, the orientational order parameter
$S_{xx}$ shows little change with even a modest increase above
$\phi=0.30$. \modify{This modest increase in $S_{xx}$ is in contrast
to the behavior of $S_{xx}$ in suspensions of homonuclear particles.
This behavior can be attributed to two causes. First is that
the increase in $S_{xx}$ comes at the expense of
orientation order along the gradient axis $S_{yy}$, which implies that
the small bump particles may not be flipping as often as
the homonuclear particles; neither, of course, flip as often as
expected from Jeffery's solution. The second cause for this observation
hinges on the fact the alignment in the vorticity direction increases
more rapidly in suspensions of homonuclear particles with increasing volume
fraction than in suspensions of small-bump particles. This more
rapid alignment with the vorticity direction in suspensions of
homonuclear particles leaves a smaller fraction to be distributed
between the flow and the gradient direction than in suspensions of
small-bump particles. This slower vorticity alignment
in suspensions of small-bump particles also contributes
to the modest increase observed in $S_{xx}$.}

The behavior of fused-dumbbells is qualitatively similar to
homonuclear particles in the low to moderate volume fraction
region, but with significantly exaggerated effects. At
$\phi=0.05$, a dramatic shift towards higher orbit constants is
seen with large positive $\Delta C_b^m $.  Upon further increase
in volume fraction, a gradual shift towards the vorticity axis
(negative $\Delta C_b^m$) is observed.  But, unlike the previous
particle shapes, the shift toward the vorticity axis and lower
orbit constants was found to essentially plateau for $0.2 \leq
\phi \leq 0.4$.  There is negligible variation in the
orientational order parameter along any of the three axes, which
is consistent with the leveling out of $\Delta C_b^m $.  At
$\phi \geq 0.5$, there is an increase in the orientational order
along the $x$ axis which comes at the expense of the
orientational order along the $y$ axis. As suggested above, this
implies that the particles at high volume fractions aren't
flipping as often as expected in Jeffery's orbits.

